External Language Model Integration for Factorized Neural Transducers

We propose an adaptation method for factorized neural transducers (FNT) with external language models. We demonstrate that both neural and n-gram external LMs add significantly more value when linearly interpolated with predictor output compared to shallow fusion, thus confirming that FNT forces the predictor to act like regular language models. Further, we propose a method to integrate class-based n-gram language models into FNT framework resulting in accuracy gains similar to a hybrid setup. We show average gains of 18% WERR with lexical adaptation across various scenarios and additive gains of up to 60% WERR in one entity-rich scenario through a combination of class-based n-gram and neural LMs.

==> fnt_tikz.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,426); %set diagram left start at 0, and has height of 426

%Rounded Rect [id:dp5395391620504593] 
\draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=0.5 ][dash pattern={on 0.84pt off 2.51pt}] (115,112.2) .. controls (115,105.79) and (120.19,100.6) .. (126.6,100.6) -- (450.4,100.6) .. controls (456.81,100.6) and (462,105.79) .. (462,112.2) -- (462,147) .. controls (462,153.41) and (456.81,158.6) .. (450.4,158.6) -- (126.6,158.6) .. controls (120.19,158.6) and (115,153.41) .. (115,147) -- cycle ;
%Rounded Rect [id:dp15219974538748282] 
\draw  [fill={rgb, 255:red, 74; green, 170; blue, 226 }  ,fill opacity=0.72 ] (124,320) .. controls (124,315.58) and (127.58,312) .. (132,312) -- (200,312) .. controls (204.42,312) and (208,315.58) .. (208,320) -- (208,344) .. controls (208,348.42) and (204.42,352) .. (200,352) -- (132,352) .. controls (127.58,352) and (124,348.42) .. (124,344) -- cycle ;
%Rounded Rect [id:dp8219155187485916] 
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (17,321) .. controls (17,316.58) and (20.58,313) .. (25,313) -- (93,313) .. controls (97.42,313) and (101,316.58) .. (101,321) -- (101,345) .. controls (101,349.42) and (97.42,353) .. (93,353) -- (25,353) .. controls (20.58,353) and (17,349.42) .. (17,345) -- cycle ;

%Rounded Rect [id:dp25444389253044464] 
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (46,235) .. controls (46,230.58) and (49.58,227) .. (54,227) -- (179,227) .. controls (183.42,227) and (187,230.58) .. (187,235) -- (187,259) .. controls (187,263.42) and (183.42,267) .. (179,267) -- (54,267) .. controls (49.58,267) and (46,263.42) .. (46,259) -- cycle ;
%Straight Lines [id:da8841591414641305] 
\draw    (59,312.6) -- (59,269.6) ;
\draw [shift={(59,267.6)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da993276542787576] 
\draw    (152,311.6) -- (152,269) ;
\draw [shift={(152,267)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da489861267861877] 
\draw    (60,375.6) -- (60,354.6) ;
\draw [shift={(60,352.6)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da744317253892504] 
\draw    (163,376.6) -- (163,355.6) ;
\draw [shift={(163,353.6)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Rounded Rect [id:dp8367863842912848] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 74; green, 180; blue, 226 }  ,fill opacity=0.65 ] (224,235.72) .. controls (224,231.46) and (227.46,228) .. (231.72,228) -- (377.28,228) .. controls (381.54,228) and (385,231.46) .. (385,235.72) -- (385,258.88) .. controls (385,263.14) and (381.54,266.6) .. (377.28,266.6) -- (231.72,266.6) .. controls (227.46,266.6) and (224,263.14) .. (224,258.88) -- cycle ;
%Straight Lines [id:da38096254303846466] 
\draw    (152,311.6) -- (271.12,268.28) ;
\draw [shift={(273,267.6)}, rotate = 160.02] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Rounded Rect [id:dp4194363126703784] 
\draw  [fill={rgb, 255:red, 184; green, 233; blue, 134 }  ,fill opacity=1 ] (172,118) .. controls (172,113.58) and (175.58,110) .. (180,110) -- (449,110) .. controls (453.42,110) and (457,113.58) .. (457,118) -- (457,142) .. controls (457,146.42) and (453.42,150) .. (449,150) -- (180,150) .. controls (175.58,150) and (172,146.42) .. (172,142) -- cycle ;
%Rounded Rect [id:dp9929578450359815] 
\draw  [fill={rgb, 255:red, 248; green, 231; blue, 28 }  ,fill opacity=1 ] (125,119) .. controls (125,114.58) and (128.58,111) .. (133,111) -- (159,111) .. controls (163.42,111) and (167,114.58) .. (167,119) -- (167,143) .. controls (167,147.42) and (163.42,151) .. (159,151) -- (133,151) .. controls (128.58,151) and (125,147.42) .. (125,143) -- cycle ;
%Straight Lines [id:da7428939865335735] 
\draw    (145,226.6) -- (145.97,153.6) ;
\draw [shift={(146,151.6)}, rotate = 90.76] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Flowchart: Or [id:dp5559980515228822] 
\draw   (346,186.8) .. controls (346,180.06) and (351.37,174.6) .. (358,174.6) .. controls (364.63,174.6) and (370,180.06) .. (370,186.8) .. controls (370,193.54) and (364.63,199) .. (358,199) .. controls (351.37,199) and (346,193.54) .. (346,186.8) -- cycle ; \draw   (346,186.8) -- (370,186.8) ; \draw   (358,174.6) -- (358,199) ;
%Straight Lines [id:da34053803142483363] 
\draw    (300,228) -- (347.32,197.68) ;
\draw [shift={(349,196.6)}, rotate = 147.35] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da7764479260363109] 
\draw    (358,174.6) -- (358,150.6) ;
\draw [shift={(358,148.6)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Rounded Rect [id:dp9815731975812454] 
\draw  [fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=1 ] (478,316.8) .. controls (478,312.38) and (481.58,308.8) .. (486,308.8) -- (554,308.8) .. controls (558.42,308.8) and (562,312.38) .. (562,316.8) -- (562,340.8) .. controls (562,345.22) and (558.42,348.8) .. (554,348.8) -- (486,348.8) .. controls (481.58,348.8) and (478,345.22) .. (478,340.8) -- cycle ;

%Straight Lines [id:da628817700204076] 
\draw    (522,370.4) -- (522,349.4) ;
\draw [shift={(522,347.4)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da4499612130965216] 
\draw    (519,308.6) -- (519,265.6) ;
\draw [shift={(519,263.6)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Rounded Rect [id:dp2366778352358403] 
\draw  [fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=1 ] (459,232.72) .. controls (459,228.46) and (462.46,225) .. (466.72,225) -- (624.28,225) .. controls (628.54,225) and (632,228.46) .. (632,232.72) -- (632,255.88) .. controls (632,260.14) and (628.54,263.6) .. (624.28,263.6) -- (466.72,263.6) .. controls (462.46,263.6) and (459,260.14) .. (459,255.88) -- cycle ;


%Straight Lines [id:da8418921795230156] 
\draw    (541,223.6) -- (369.97,195.92) ;
\draw [shift={(368,195.6)}, rotate = 9.19] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da7545318325232577] 
\draw    (274,99.6) -- (274,68.6) ;
\draw [shift={(274,66.6)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da10698954407555705] 
\draw    (541,223.6) -- (540.02,105.6) ;
\draw [shift={(540,103.6)}, rotate = 89.52] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Rounded Rect [id:dp9771750126406995] 
\draw  [dash pattern={on 0.84pt off 2.51pt}] (446,244.4) .. controls (446,222.97) and (463.37,205.6) .. (484.8,205.6) -- (602.2,205.6) .. controls (623.63,205.6) and (641,222.97) .. (641,244.4) -- (641,360.8) .. controls (641,382.23) and (623.63,399.6) .. (602.2,399.6) -- (484.8,399.6) .. controls (463.37,399.6) and (446,382.23) .. (446,360.8) -- cycle ;

% Text Node
\draw (24,323.4) node [anchor=north west][inner sep=0.75pt]    {$predictor_{\phi }$};
% Text Node
\draw (96.52,237.4) node [anchor=north west][inner sep=0.75pt]    {$joint_{\phi }$};
% Text Node
\draw (35,282.4) node [anchor=north west][inner sep=0.75pt]    {$g_{u}^{\phi }$};
% Text Node
\draw (132,284.4) node [anchor=north west][inner sep=0.75pt]    {$f_{t}$};
% Text Node
\draw (49,382.4) node [anchor=north west][inner sep=0.75pt]    {$y_{1}^{u}$};
% Text Node
\draw (153,381.4) node [anchor=north west][inner sep=0.75pt]    {$x_{1}^{t}$};
% Text Node
\draw (134,119.4) node [anchor=north west][inner sep=0.75pt]    {$z_{t,u}^{\phi }$};
% Text Node
\draw (300,195.4) node [anchor=north west][inner sep=0.75pt]    {$z_{t}^{v}$};
% Text Node
\draw (139,324.4) node [anchor=north west][inner sep=0.75pt]    {$encoder$};
% Text Node
\draw (485,319.2) node [anchor=north west][inner sep=0.75pt]    {$predictor_{V}$};
% Text Node
\draw (442,183.4) node [anchor=north west][inner sep=0.75pt]    {$z_{u}^{v}$};
% Text Node
\draw (222,117.4) node [anchor=north west][inner sep=0.75pt]    {$z_{t,u}^{v} :\ vocabulary\ scores$};
% Text Node
\draw (224,41.4) node [anchor=north west][inner sep=0.75pt]    {$P\left(\hat{y}_{t+1} |x_{1}^{t} ,y_{1}^{u}\right)$};
% Text Node
\draw (493,75.4) node [anchor=north west][inner sep=0.75pt]    {$z_{u}^{v} =log\ P\left( y_{u+1} |y_{1}^{u}\right)$};
% Text Node
\draw (232,236.4) node [anchor=north west][inner sep=0.75pt]    {$log\ \sigma \left( W_{enc}^{V} \cdot relu( f_{t})\right)$};
% Text Node
\draw (516,158.4) node [anchor=north west][inner sep=0.75pt]    {$z_{u}^{v}$};
% Text Node
\draw (468.72,228.4) node [anchor=north west][inner sep=0.75pt]    {$log\ \sigma \left( W_{pred}^{V} \cdot relu\left( g_{u}^{v}\right)\right)$};
% Text Node
\draw (511,377.2) node [anchor=north west][inner sep=0.75pt]    {$y_{1}^{u}$};
% Text Node
\draw (498,276.4) node [anchor=north west][inner sep=0.75pt]    {$g_{u}^{v}$};
% Text Node
\draw (429.75,383.97) node [anchor=north west][inner sep=0.75pt]  [rotate=-270.19] [align=left] {\textit{Pretrained external LM}};


\end{tikzpicture}

